Vertex-based Networks to Accelerate Path Planning Algorithms

Path planning plays a crucial role in various autonomy applications, and RRT* is one of the leading solutions in this field. In this paper, we propose the utilization of vertex-based networks to enhance the sampling process of RRT*, leading to more efficient path planning. Our approach focuses on critical vertices along the optimal paths, which provide essential yet sparser abstractions of the paths. We employ focal loss to address the associated data imbalance issue, and explore different masking configurations to determine practical tradeoffs in system performance. Through experiments conducted on randomly generated floor maps, our solutions demonstrate significant speed improvements, achieving over a 400% enhancement compared to the baseline model.

==> conclusion.tex <==
\chapter{Conclusions}
This thesis introduced a new hybrid training technique that is implemented under NengoDL and compared its performance against equivalent ANN models. 
Furthermore, this thesis was able to provide more insight into the estimated energy consumption between ANNs and SNNs.
As mentioned in the results section, the hybrid neurons were able to be used under NengoDL using the two main techniques to manipulate firing rates: firing rate scaling and firing rate regularization. 
However, more experiments should be tested using the firing rate scaling method on the hybrid neurons due to the results stated in section \ref{sec:obj_loc}.
Due to the simplicity of both networks, future work should attempt to apply the hybrid training phase and neurons to larger networks with different data.
This would ensure that they can be applied to those networks under NengoDL, and possibly outside of NengoDL as well. 
Continuing with NengoDL, the hybrid neurons were only implemented for the Rectified Linear and soft LIF neurons. 
Using algorithm \ref{alg:hybrid}, future work could include hybrid neurons for other neurons available through Nengo and NengoDL.

One of the larger limitations of this work is that it is only done through an SNN simulator using NengoDL. 
This simulator uses the CPU and/or GPU in order to run the SNN for inference.
A valuable asset to Nengo and NengoDL is its ability to be run on neuromorphic hardware such as Intel's Loihi neuromorphic chip.
At the current time, object localization and image segmentation models have been run using the NengoLoihi simulator which simulates using the Loihi chip on a CPU or GPU. 
However, such models have not gone through a hybrid training phase using hybrid neurons. 
This is because the NengoLoihi neurons are built differently than the Nengo and NengoDL neurons so modifications would have to be made in order for them to work. 
Additionally, a large quantization error starts to occur between Nengo/NengoDL neurons and NengoLoihi neurons after the firing rates reach above 300 Hz. 
Knowing this, the models would have to be retrained with that firing rate in mind to ensure that they can perform well using NengoLoihi. 
Finally, permission must be granted to use the actual Loihi chip provided by Intel. 
With this permission, one could use NengoLoihi and deploy their model to the hardware itself and run the SNN model. Currently we are in this process but we are unsure when it will be completed.
Deploying the hybrid trained models onto neuromorphic hardware via NengoLoihi would make certain that the hybrid training phase increases performance of SNN models in the general case as well as providing a lower energy consumption when compared to equivalent ANN models.



==> exp.tex <==

\chapter{Introduction}
\vspace{1in}
\vspace{1in}
\vspace{1in}


\section{Artificial Neural Networks}


\vspace{1in}
\vspace{1in}
\vspace{1in}

\section{Spiking Neural Networks}

\vspace{1in}
\vspace{1in}
\vspace{1in}


\section{Spiking Neural Network Optimization}

\vspace{1in}
\vspace{1in}
\vspace{1in}


\section{Thesis Contributions and Overview}

\vspace{1in}
\vspace{1in}
\vspace{1in}






==> timeline.tex <==

\chapter{Timeline}
The period of the proposed plan is 12 months, which is divided into the following milestones:

\begin{itemize}
\item September 2022-December 2022: Implement the vertex objective network accelerated RRT*.
\item January 2023-Feburary 2023: Finish the experiment result of vertex objective network accelerated RRT*, write the paper for this work and submit for publication.
\item March 2023-May 2023: Develop the transformer accelerated RRT*.
\item September 2023-October 2023: Write the paper for transformer accelerated RRT* and submit it to a conference.
\item October 2023-December 2023: Complete the dissertation and proceed with the dissertation defense.
\end{itemize}




